Casablanca: Data and Models for Multidialectal Arabic Speech Recognition

In spite of the recent progress in speech processing, the majority of world languages and dialects remain uncovered. This situation only furthers an already wide technological divide, thereby hindering technological and socioeconomic inclusion. This challenge is largely due to the absence of datasets that can empower diverse speech systems. In this paper, we seek to mitigate this obstacle for a number of Arabic dialects by presenting Casablanca, a large-scale community-driven effort to collect and transcribe a multi-dialectal Arabic dataset. The dataset covers eight dialects: Algerian, Egyptian, Emirati, Jordanian, Mauritanian, Moroccan, Palestinian, and Yemeni, and includes annotations for transcription, gender, dialect, and code-switching. We also develop a number of strong baselines exploiting Casablanca. The project page for Casablanca is accessible at: www.dlnlp.ai/speech/casablanca.

==> Sections/Baseline_models/ADI.tex <==
% \subsection{Arabic Dialect Identification (ADI)}

==> Sections/Baseline_models/SER.tex <==
% \mam{Edit this small paragraph.} 
% Speech Emotion Recognition (SER) identifies emotions in spoken language, crucial for human-computer interaction. It deals with classifying specific emotions or assessing them on scales like valence and arousal. However, SER is challenged by the scarcity of diverse datasets, with notable examples like IEMOCAP and CMU-MOSEI primarily in English, highlighting the need for more varied emotional speech data. We provide more detailed coverage of emotion in speech in Appendix \ref{app:ser}.
% 
% For Arabic emotion datasets, the landscape significantly diverges from that of English. The majority of work in developing emotion datasets was devoted to training a particular model for evaluation purposes. Subsequently, these databases are often not made open-source or may even become inaccessible. Among the few available datasets for Arabic SER, KSUEmotions \cite{KSUEMOTIONS} stands out as the current benchmark, with only a handful of others accessible. This acted database offers five hours of recordings balanced by gender, featuring 13 female and 10 male speakers with five labels (Neutral, angry, sad, happy, and surprised). However, KSUEmotions faces two primary challenges. Firstly, it is not entirely open-source, being available commercially for a fee, which limits its accessibility for broader research and development efforts. Secondly, the dataset is criticized for its heavily scripted nature, featuring only 16 sentences that are repeated by all speakers across different emotions. This aspect raises concerns about the dataset's realism and its applicability in creating emotion recognition systems that can effectively handle the nuances of natural speech. Another Arabis dataset that is freely accessible is the Arabic Natural Audio Dataset (ANAD)\cite{ANAD}, which consists of eight videos capturing live calls between an anchor and a person outside the studio taken from Arabic talk shows. These were segmented into 1,384 one-second clips, each annotated with one of three labels (Happy, Angry, and Surprised). The primary issue with ANAD, however, is its limited size, which constrains its utility for training large-scale SER models.
\textbf{Arabic emotion data.}
% Speech Emotion Recognition (SER) identifies emotions in spoken language, essential for enhancing human-computer interaction by classifying emotions or assessing them on scales such as valence and arousal. Despite its potential, SER faces challenges due to the limited diversity of datasets, with notable English datasets like IEMOCAP and CMU-MOSEI underscoring the need for more varied emotional speech data. 
Speech Emotion Recognition (SER) identifies emotions in spoken language, crucial for enhancing human-computer interaction by classifying emotions or assessing them on scales such as valence and arousal. Despite its potential, SER is limited by a predominant focus on English datasets~\cite{IEMOCAP, CMUMOSEI}, highlighting the need for more diverse and multilingual emotional speech data.
% Further details are available in Appendix \ref{app:ser}.\todo{It is not common/acceptable to use the appendix for related work } 
% In Arabic SER, the landscape is markedly different, with most datasets developed for specific model training, resulting in limited public availability. Among the few, KSUEmotions \cite{KSUEMOTIONS} is a benchmark, offering five hours of recordings from 13 female and 10 male speakers, covering five emotions. Despite its value, KSUEmotions is commercially available, limiting wider access, and is critiqued for its scripted content from 16 sentences, questioning its real-world applicability. Another dataset, the Arabic Natural Audio Dataset (ANAD) \cite{ANAD}, freely available, includes 1,384 one-second clips from eight videos, annotated with three emotions. However, ANAD's small size limits its utility for training comprehensive SER models.
In Arabic SER, the landscape is distinct, with many datasets tailored for specific model training and limited public availability. KSUEmotions \cite{KSUEMOTIONS}, a notable example, offers five hours from 13 female and 10 male speakers covering five emotions. However, its commercial nature restricts access, and its scripted content from only 16 sentences does not reflect real-world scenarios. The Arabic Natural Audio Dataset (ANAD) \cite{ANAD}, freely available, includes 1,384 one-second clips from eight videos, annotated with three emotions, but its small size hampers its effectiveness for comprehensive SER model training.














==> Sections/Baseline_models/SER_experiments_appendex.tex <==
\subsection{SER Experiments details}

\label{EXP details}
\begin{table}[h!]
\centering
\tiny
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lccc}
\hline
\textbf{Experiment} & \textbf{Train}       &  \textbf{Validation} &  \textbf{Test} \\ \hline

\textbf{Experiment 1}     & 10048 (11.3)        & 1257 (1.5)  & 1256 (1.5) \\ 

\textbf{Experiment 2}   & 6798 (7.7)       & 850 (0.8) & 850 (1.0) \\

\textbf{Experiment 3}       & 8662 (9.9)          & 1083 (1.1) & 1083 (1.3) \\ 

\end{tabular}%
}
\caption{The number of data points (hours) in the train, test, and validation splits in the SER Experiments.}
\label{tab:SER Experiments details}
\end{table}
Table \ref{tab:SER Experiments details} shows the train, test, and validation split used in each experiment. We acknowledge that our dataset annotated for SER is imbalanced, and we intend to address this problem by adding more annotations in the future.  For all three experiments, we use the current state-of-the-art architecture for speech emotion recognition inspired by \cite{SER_SOTA}, utilizing Hubert (base) \cite{hubert} as the encoder and adding a simple average pooling layer followed by a feed-forward neural network head on top for projection and classification. We fine-tune the whole model except for the feature extractor (CNN) layer in Hubert using a learning rate of 0.001 and a batch size of 64 on an A100 GPU.


==> Sections/Baseline_models/ST.tex <==
\subsection{Emotion Recognition}

% For emotion recognition, we carry out experiments under two main
% settings. Setting one has two stages and setting two has one stage. 

% \textbf{Setting one:} Two stage, where we \textbf{first} tease apart the emotion carrying data from the neutral class, \textbf{then} classify the emotion carrying segments into their exact emotion label. 

% \textbf{Setting two:} We also remove the "other" class and develop a classifier exploiting the data (6 classes, including neutral). 

% We develop models based on w2v as well as HuBERT. 

\noindent In the Speech Emotion Recognition (SER) task, we conduct three experiments:

\textbf{Experiment-1}: Initially, we execute a binary classification task by categorizing the emotions  \textit{Angry},  \textit{Other},  \textit{Sad},  \textit{Happy},  \textit{Surprised},  \textit{Disgusted}, and  \textit{Fearful} into a group that signifies active emotions. Conversely, the emotion  \textit{Neutral} is categorized as the passive emotion class. This initial experiment plays a crucial role, as differentiating between expressive and subdued emotions holds significant implications for enhancing interactions between humans and computers. Table \ref{tab:Emotions Experiments results} details the outcomes of this \textbf{Binary} experiment. While acknowledging the limitations of unbalanced data, these results still provide valuable insights and can act as a baseline for future work.

%%%%%%%%
\begin{table}[h!]
\centering
\tiny
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{lccc}
\hline
\textbf{Experiment} & \textbf{F1 score}       &  \textbf{WA} &  \textbf{UAR}\\ \hline

\textbf{Binary}     & 0.69        & 68.9\% & - \\ 

\textbf{Multiclass 4 labels}   & \textbf{0.58}       & \textbf{58.2}\% & \textbf{53.2} \\


\textbf{Multiclass 7 labels}       & 0.35          & 33.6\% &  33.1\\ \hline


\end{tabular}%
}
\caption{Baseline results in SER for ~\ourdataset. \textit{"WA"}: (Weighted Accuracy) the classiﬁcation accuracy weighted by whole test set. \textit{"UAR"}: (Unweighted Average Recall) calculates the Recall for each label, then find their unweighted means.}
\label{tab:Emotions Experiments results}
\end{table}


\textbf{Experiment-2}: In the second experiment, we performed a standard multiclass speech emotion recognition using the following classes: Angry, Sad, Happy, and Neutral. Those labels are considered the standard for benchmarking SER datasets \cite{SER_SOTA,SER2,SER3,IEMOCAP}. The results for this experiment is shown in Table \ref{tab:Emotions Experiments results} we intend for those results to act as the main baseline for the SER portion of our dataset. 

\textbf{Experiment-3}: In the Third experiment, we performed a multiclass speech emotion recognition using most of the classes including: Angry, Sad, Happy, Surprised, Disgusted, Fearful, and Neutral. We excluded the 'Other' class, as it is an ambiguous label typically used by annotators when they are unable to clearly identify the emotion being expressed. The results for this experiment are also shown in Table \ref{tab:Emotions Experiments results}


\noindent For all three experiments we use the current state of the art architecture for speech emotion recognition inspired by \cite{SER_SOTA}, utilising Hubert as the encoder and adding a simple feed forward neural network head on top for projection and classification. More information about the setup for the three experiments could be found in appendix \ref{EXP details}.





% \textit{\textbf{Maybe skip ST...}}



==> Sections/Corpus_Collection/Data_Filtering.tex <==
\subsection{Data Filtering}

- Automatic Filtering \textcolor{red}{\textbf{(After segmentation)}}\\
\noindent
- Manual Filtering \textcolor{red}{\textbf{(During annotation})}

\\

[MOVE THIS TO DATA SEGMENTATION]
- we removed utterances that are shorter than 3 seconds to avoid short utterances as participants will select segments from these utterances.

[MOVE THIS TO DATA ANNOTATION]
- Split the data (we didn't use all of the series. I remember we used 3 episodes.. check the "Import" dir in the annotation.).

All details and examples

\textbf{Narrative as a story}

Visualization of pipeline

==> Sections/Data_Annotation/Annotation_tool.tex <==
\subsection{Annotation Tool}
\label{sec-annotation-tool}
% \DONE{Bashar}{For our choice of annotation tool, w}
We employed \textit{Label-Studio}\footnote{\href{https://labelstud.io/}{https://labelstud.io/}}, a widely supported open-source labeling platform, as our choice for an annotation tool. We centrally hosted it on our servers and provided online access, allowing for remote and adaptable involvement from annotators across various locations. 
\INPROGRESS{Note}{transcript is the written document that results from the transcription process}
Within the tool we used the `\textit{Automatic Speech Recognition using Segments}' template \footnote{ \href {https://labelstud.io/templates/automatic_speech_recognition_segments}{https://labelstud.io/templates/automatic\_speech\_recognition\_segments}}, enabling annotators to select multiple spans from each snippet and write their transcriptions accompanied by additional metadata. We also customized the tool to allow annotators to specify the gender of the speaker for each segment. 
% To maintain an organized workflow, we established a sub-project for each dialect and uploaded all corresponding snippets under these specific sub-projects. 
% To ensure the independence of each snippet from its preceding and following counterparts, we randomly shuffled the data. This strategy was crucial in eliminating potential biases or sequencing effects in the annotation process where the order in which data is presented could influence the annotator's perception or interpretation. \\
We randomly shuffled the data to guarantee each snippet's independence, effectively reducing potential bias and sequencing effects that could impact annotators' perceptions during the annotation process.
% \DONE{Bashar}{I think we have to elaborate more about what we're trying to avoid. From my understanding working on the project, we want to avoid inferring what is being said from context obtained from a previous or subsequent conversation so we don't expect that from the model. But I'm not sure it's clear for someone outside of the project.}
% \textcolor{purple}{\small I think we have to elaborate more about what we're trying to avoid. From my understanding working on the project, we want to avoid inferring what is being said from context obtained from a previous or subsequent conversation so we don't expect that from the model. But I'm not sure it's clear for someone outside of the project.}\\

% \noindent
% The tool also provides annotators with the functionality to sort and search for snippets using various parameters such as ID, annotator name, modified date, content, among others. This feature enhances the ease of navigation and management of the data. Although we have restricted the ability of annotators to upload data, they retained the option to skip any snippet. Additionally, the tool's capability to export labeled data in a \texttt{JSON} format allows for straightforward integration of the labled data into our speech models.


% The tool allows us to export a \texttt{JSON} file that has all the labeled data that can be parsed and directly integrated into our speech models.



==> Sections/Data_Annotation/Annotation_tool_2.tex <==
\subsection{Annotation Tool}
\label{sec-annotation-tool}
% \DONE{Bashar}{For our choice of annotation tool, w}
We employed \textit{Label-Studio}\footnote{\href{https://labelstud.io/}{https://labelstud.io/}}, a widely supported open-source labeling platform, as our choice for an annotation tool. We centrally hosted it on our servers and provided online access, allowing for remote and adaptable involvement from annotators across various locations. 
\INPROGRESS{Note}{transcript is the written document that results from the transcription process}
Within the tool we used the `\textit{Automatic Speech Recognition using Segments}' template \footnote{ \href {https://labelstud.io/templates/automatic_speech_recognition_segments}{https://labelstud.io/templates/automatic\_speech\_recognition\_segments}}, enabling annotators to select multiple spans from each snippet and write their transcriptions accompanied by additional metadata. We also customized the tool to allow annotators to specify the gender of the speaker for each segment. 
% To maintain an organized workflow, we established a sub-project for each dialect and uploaded all corresponding snippets under these specific sub-projects. 
% To ensure the independence of each snippet from its preceding and following counterparts, we randomly shuffled the data. This strategy was crucial in eliminating potential biases or sequencing effects in the annotation process where the order in which data is presented could influence the annotator's perception or interpretation. \\
We randomly shuffled the data to guarantee each snippet's independence, effectively reducing potential bias and sequencing effects that could impact annotators' perceptions during the annotation process.
% \DONE{Bashar}{I think we have to elaborate more about what we're trying to avoid. From my understanding working on the project, we want to avoid inferring what is being said from context obtained from a previous or subsequent conversation so we don't expect that from the model. But I'm not sure it's clear for someone outside of the project.}
% \textcolor{purple}{\small I think we have to elaborate more about what we're trying to avoid. From my understanding working on the project, we want to avoid inferring what is being said from context obtained from a previous or subsequent conversation so we don't expect that from the model. But I'm not sure it's clear for someone outside of the project.}\\

% \noindent
% The tool also provides annotators with the functionality to sort and search for snippets using various parameters such as ID, annotator name, modified date, content, among others. This feature enhances the ease of navigation and management of the data. Although we have restricted the ability of annotators to upload data, they retained the option to skip any snippet. Additionally, the tool's capability to export labeled data in a \texttt{JSON} format allows for straightforward integration of the labled data into our speech models.


% The tool allows us to export a \texttt{JSON} file that has all the labeled data that can be parsed and directly integrated into our speech models.



==> Sections/Dialects_Description/Dialects_Description_2.tex <==
\section{Dialects Description}
% We introduce
\label{sec:dialect-desc}
% \ourdataset is a comprehensive and meticulously annotated dataset encompassing a diverse array of eight distinct Arabic dialects, representing various regions across the Arab world, including the Levantine area, the Gulf region, Yemeni, and North African countries. The total duration of the dataset is $\approx$ 48 hours. The dialects featured in our dataset are Egyptian, Jordanian, Palestinian, Emirati, Algerian, Moroccan, Mauritanian (Hassaniya), and Yemeni. Each dialect is distinct, reflecting the unique linguistic characteristics of its respective region and maintaining the non-standard orthographic features of each dialect. Delving deeper into the linguistic intricacies of our dataset, we highlight the sub-dialects found within the series of each primary dialect, showcasing the rich tapestry of linguistic variations in our dataset. The sub-dialects are identified by the native speakers of each respective dialect to ensure their accuracy. A detailed description of the identified sub-dialects is presented in Appendix~\ref{sec:appendix}. One of \ourdataset's main contributions lies in its inclusion of newly annotated data for Mauritanian, Emirati, and Yemeni dialects. To the best of our knowledge, Casablanca is the first dataset to cover both low- and zero-resourced dialects, specifically the aforementioned dialects, thus filling a significant need in the research landscape. These dialects have been notably underrepresented in research, primarily focusing on morphologically annotated corpora of the Yemeni dialect, which is part of a broader focus on seven Arabic dialects,~\cite{alshargi2019morphologically}, including Taizi and Sanaani.



\ourdataset~is a detailed collection of around 48 hours of data covering eight Arabic dialects from regions like the Levant, Gulf, Yemen, and North Africa, including Algerian, Egyptian, Emirati, Jordanian, Mauritanian (Hassaniya), Moroccan, Palestinian, and Yemeni.
% \mam{List the regions and the dialects in alphabetical order. Follow this in anything you would like to list, unless you have other reasons not to.} 
% \DONE{Bashar}{Done. This is what I did in the tables.}
\ourdataset~involves sub-dialects from these countries as well. In addition, to the best of our knowledge, we are among the first to offer annotated data for the less-represented Emirati, Mauritanian, and Yemeni dialects, addressing a gap in linguistic research. 



























% The study of Arabic dialects reveals many distinctive linguistic variations across different levels, such as syntax, semantics, phonology, and morphology—our annotated data endeavors to meticulously identify specific sub-dialects within each principal dialect. 
% \noindent


==> Sections/Results/Results.tex <==
\section{Results}
\subsection{ASR results}


For the first scenario in \textit{\textbf{dialects evaluation}}, we report WER and CER of four different multilingual models on the eight novel dialects, which we hypothesize may not have been incorporated into the training data of these models. As shown in Table~\ref{x}, all models exhibited high WER and CER across each dialect, indicating their inability to effectively generalize to entirely novel conditions. On average, \textit{whisper-large-v3} recorded lower WER and CER compared to other models, both with preprocessing (69.49 WER and 31.16 CER) and without (63 WER and 28.17 CER). In terms of dialects, without any preprocessing, only the Jordanian dialect achieved a WER of less than 50, as recorded by both Whisper models and SeamlessM4T. After preprocessing, the Palestinian and Egyptian dialects approached a WER of around 50 with these models. 




% \begin{table*}[]
% \resizebox{\textwidth}{!}{%

% \begin{tabular}{lllllllll}
%  & \multicolumn{2}{l}{whisper-msa} & \multicolumn{2}{l}{whisper-mixed} & \multicolumn{2}{l}{whisper-egyptian} & \multicolumn{2}{l}{whisper-moroccan} \\
%            & WER        & CER         & WER      & CER     & WER     & CER     & WER     & CER     \\
% Algeria    & 87.86      & 48.31       & 129.63\% & 79.63\% & 86.68\% & 35.80\% & 74.39\% & 29.50\% \\
% Egypt      & 67.68      & 35.22       & 97.31\%  & 63.87\% & 49.58\% & 19.33\% & 74.82\% & 34.83\% \\
% Jordan     & 61.19\%    & 23.44\%     & 78.15\%  & 40.34\% & 56.11\% & 18.15\% & 72.79\% & 27.12\% \\
% Mauritania & 88.02      & 47.5        & 114.39\% & 78.02\% & 87.08\% & 43.32\% & 89.93\% & 45.16\% \\
% Morocco    & 88.06      & 46.37       & 120.59\% & 77.44\% & 84.85\% & 37.22\% & 61.58\% & 21.25\% \\
% Palestine  & 68.06\%    & 28.90\%     & 76.92\%  & 36.81\% & 63.70\% & 22.31\% & 76.83\% & 30.15\% \\
% UAE        & 74.24\%    & 35.38\%     & 104.60\% & 60.20\% & 67.45\% & 24.48\% & 78.37\% & 31.51\% \\
% Yemen      & 74.71\%    & 36.09\%     & 96.01\%  & 54.81\% & 70.49\% & 28.07\% & 79.13\% & 33.89\% \\
% AVG        & 41.8002482 & 22.32975711 & 102.20\% & 61.39\% & 70.74\% & 28.58\% & 75.98\% & 31.68\%
% \end{tabular}
% }
% \end{table*}

% \begin{table*}[]
% \resizebox{\textwidth}{!}{%

% \begin{tabular}{lcccc}
% \hline
% \textbf{} &
%   \textbf{whisper-msa} &
%   \textbf{whisper-mixed} &
%   \textbf{whisper-egyptian}&
%   \textbf{whisper-moroccan}\\ \hline
% Algeria    & (87.86/48.31)   & (129.63, /79.63, ) & (86.68, /35.80, ) & (74.39, /29.50, ) \\
% Egypt      & (67.68/35.22)   & (97.31, /63.87, ) & (49.58, /19.33, ) & (74.82, /34.83, ) \\
% Jordan     & (61.19, /23.44, ) & (78.15, /40.34, ) & (56.11, /18.15, ) & (72.79, /27.12, ) \\
% Mauritania & (88.02/47.5)    & (114.39, /78.02, ) & (87.08, /43.32, ) & (89.93, /45.16, ) \\
% Morocco    & (88.06/46.37)   & (120.59, /77.44, ) & (84.85, /37.22, ) & (61.58, /21.25, ) \\
% Palestine  & (68.06, /28.90, ) & (76.92, /36.81, ) & (63.70, /22.31, ) & (76.83, /30.15, ) \\
% UAE        & (74.24, /35.38, ) & (104.60, /60.20, ) & (67.45, /24.48, ) & (78.37, /31.51, ) \\
% Yemen      & (74.71, /36.09, ) & (96.01, /54.81, ) & (70.49, /28.07, ) & (79.13, /33.89, ) \\
% AVG        & (41.80/22.32)   & (102.20, /61.39, ) & (70.74, /28.58, ) & (75.98, /31.68, ) \\ \hline
% \end{tabular}
% }
% \end{table*}


